On-Device Bug Reporting for Android Applications

Bugs that surface in mobile applications can be difficult to reproduce and fix due to several confounding factors including the highly GUI-driven nature of mobile apps, varying contextual states, differing platform versions and device fragmentation. It is clear that developers need support in the form of automated tools that allow for more precise reporting of application defects in order to facilitate more efficient and effective bug fixes. In this paper, we present a tool aimed at supporting application testers and developers in the process of On-Device Bug Reporting. Our tool, called ODBR, leverages the uiautomator framework and low-level event stream capture to offer support for recording and replaying a series of input gesture and sensor events that describe a bug in an Android application.

==> concl.tex <==
% !TEX root = main.tex

In this demo we have presented \textbf{ODBR} a tool for efficiently and effectively capturing on-device bug reports for Android apps.  This tool is an Android app used for recording bug reports, complete with user event and GUI information, and a Java web application capable of displaying and managing bug reports collected from devices.  In the future, the bug reporting application could be further built out to incorporate system level performance information, such as CPU or memory usage. Additionally, the Java web application could be further developed to support additional features commonly found in modern day issue trackers such as issue labels, discussions, and references to code and design artifacts.

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }


\newcommand\KEVIN[1]{\nb{\color{blue}KEVIN}{#1}}
\newcommand\RICHIE[1]{\nb{\color{blue}RICHIE}{#1}}
\newcommand\DENYS[1]{\nb{\color{blue}DENYS}{#1}}
\newcommand\CARLOS[1]{\nb{\color{blue}CARLOS}{#1}}

\newcommand\NEW[1]{\nb{NEW}{#1}}






==> study.tex <==
% !TEX root = main.tex


